Step Out and Seek Around: On Warm-Start Training with Incremental Data

Data often arrives in sequence over time in real-world deep learning applications such as autonomous driving. When new training data is available, training the model from scratch undermines the benefit of leveraging the learned knowledge, leading to significant training costs. Warm-starting from a previously trained checkpoint is the most intuitive way to retain knowledge and advance learning. However, existing literature suggests that this warm-starting degrades generalization. In this paper, we advocate for warm-starting but stepping out of the previous converging point, thus allowing a better adaptation to new data without compromising previous knowledge. We propose Knowledge Consolidation and Acquisition (CKCA), a continuous model improvement algorithm with two novel components. First, a novel feature regularization (FeatReg) to retain and refine knowledge from existing checkpoints; Second, we propose adaptive knowledge distillation (AdaKD), a novel approach to forget mitigation and knowledge transfer. We tested our method on ImageNet using multiple splits of the training data. Our approach achieves up to $8.39\%$ higher top1 accuracy than the vanilla warm-starting and consistently outperforms the prior art with a large margin.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% A significant open problem in deploying deep learning models in industry is enabling neural networks to learn from dynamic streams of data incrementally. For instance, in autonomous driving, we want to improve the accuracy of a perception model systematically and efficiently as we obtain new training data~\cite{caccia2022anytime}. Learning incrementally with new data has two main challenges. On the one hand, when trained on newly arrived data, models tend to lose the previously acquired capabilities. On the other hand, as our goal is to improve the model, we must carefully select the previously acquired knowledge we want to retain. Therefore, we must find a balance between forgetting and retaining information efficiently.

\begin{figure}
    \centering
    %\includegraphics[width=0.48\linewidth]{figures/train_cost.eps}
    \includegraphics[width=\linewidth]{figures/train_cost2.eps}
    \caption{Accumulated training and storage costs as a function of the training strategy when training data is progressively available. Warm start involves using previously trained models and therefore increases the training costs. The goal here is to have fixed training and storage costs. That is, train a new model using existing models as initialization (warm-start) and only accessing to new data only.}
    \label{fig:train-cost}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\linewidth]{figures/train_cost.eps}
%     \includegraphics[width=0.48\linewidth]{figures/train_cost2.eps}
%     \caption{The accumulated training cost with different training strategies as data arrives in sequence. \red{which one is better?}}
%     \label{fig:train-cost}
% \end{figure}
An open problem in deploying deep learning models in industry is enabling neural networks to learn incrementally from dynamic streams of data. For instance, in autonomous driving, we want to improve the accuracy of a perception model systematically and efficiently as we obtain new training data~\cite{caccia2022anytime}. Continual learning also called life-long or incremental learning, is the field of research focused on developing techniques and architectures that enable deep models to learn sequentially without needing to retrain them from scratch whenever new data is available. The academic setting usually focuses on incrementally learning different tasks~\cite{mallya2018packnet, sun2023decoupling}, continuously adapting to new domain data~\cite{garg2022multi}, or when we want to increment the number of categories/objects the model can detect~\cite{luo2023class, sun2023decoupling}. In industry, however, the need is slightly different. We want a model to systematically leverage any new training data for a fixed task and architecture to improve accuracy. The straightforward approach to using this data is to train the model from scratch with all available data. However, over time, this leads to prohibitive training costs, and it is impractical in storage-limited systems where storing all past data is not feasible. Here, we focus on developing efficient algorithms to update an existing model to boost their accuracy using newly available data. % enabling incorporating new data into a trained model to boost his accuracy without training the model from scratch using all the data.

%use new data and previous models to boost the accuracy of a model without training it from scratch.  








%% this might be rephrased somewhere here
Many continual learning methods have been proposed to mitigate forgetting~\cite{de2021continual, zhou2023deep}.
However, existing continual learning approaches mostly aim at task-incremental or class-incremental situations~\cite{wu2019large, kirkpatrick2017overcoming, gao2023unified, yan2021dynamically, luo2023class}, and we empirically find that they fail to work well in the data-incremental setup which has been rarely explored. This is intuitively explainable: In class or task incremental problems, the model has converged fully on previous classes as it assumes all the related data samples are provided at once in the corresponding round.

%% This should also be early on
The data collected in the past can be accessible or not accessible in different practical applications. In storage-limited systems with no access to past data, the model suffers severe catastrophic forgetting when training on new data. 


Incrementally improving the accuracy of a model with new domain data has two main challenges. First is catastrophic forgetting; models tend to lose the previously acquired capabilities when trained on newly arrived data. Second, we must carefully select the previously acquired knowledge we want to retain. Therefore, we must find a balance between forgetting and retaining information efficiently.

In this paper, we first propose FeatReg, a novel feature regularization approach able to retain knowledge and refine the existing feature representation. 

%we propose to first step out of the previous convergence point and seek a better one. This actually also aligns with the effect of methods proposed in prior literature for model generalization improvement~\cite{ash2020warm, ramkumar2023learn, zhou2022fortuitous}, where they select heritage partial of learned knowledge allowing a better loss landscape exploration. 

Then we propose to apply a novel feature regularization (FeatReg) to retain knowledge and refine the learned feature representation in both scenarios where the past data is accessible and not accessible. For the latter scenario, we also propose to apply adaptive knowledge distillation (AdaKD) for knowledge transfer from the weak teacher.

Warm-start is a widely used approach to reducing training costs, where the model is initialized using the previous checkpoint and trained using the new data available. However, warm-start tends to hurt generalization compared to random initialization~\cite{ash2020warm, achille2017critical, caccia2022anytime}. 

Among the existing methods, inheriting selective learned knowledge from the learned model during initialization~\cite{ash2020warm, ramkumar2023learn, taha2021knowledge, zhou2022fortuitous} and adding certain regularizations~\cite{shon2022dlcft} are the most popular and have shown efficacy for accuracy improvement. 



%% One quick paragraph on regularlization and warm start- EWC?
So typical methods aim at staying as close as possible to the prior solution~\cite{kirkpatrick2017overcoming}. However, in general data-incremental, the accuracy of all classes has potential to improve given more data samples, thus requiring the model to move away from the previous convergence point learned from limited data and seek a trade-off between learning and forgetting. 

%%One short paragraph about exising methods for knowledge distillation
Knowledge distillation~\cite{gou2021knowledge} is also one of the widely applied approaches to transfer the learned knowledge to the model being trained~\cite{madaan2023heterogeneous, iscen2020memory, li2017learning, dhar2019learning}. In the data-incremental case, however, the previously trained models tend to be weak teachers as they are trained with less data. This poses additional challenges to the knowledge transfer so that the teacher does not over-guide the student~\cite{lee2023study}.



We test our algorithm with large-scale dataset ImageNet~\cite{imagenet} and show the efficacy of our method. For example in the ImageNet $10$-split case where old data is inaccessible, our method yields $8.39\%$ higher accuracy than simply warm-starting the model.
We also show that our method is compatible with other orthogonal approaches and the combination brings higher accuracy. 
\textcolor{red}{Something more specific here about numbers?}
By combining with iCaRL~\cite{rebuffi2017icarl}, a replay-based continual learning method, the accuracy is further boosted by $1.68\%$ and is $7.92\%$ higher compared to applying iCaRL only.
% and $10.07\%$ higher than simply warm-starting the model.






% % Recent advancements in machine learning have seen the potential of neural networks matching or even exceeding human-level performance in many tasks. 
% Applying machine learning algorithms to real-world applications could face challenges as the data in practice is typically not static but sequentially arrives in chunks, which violates the general assumptions of i.i.d observations~\cite{caccia2022anytime}. This requires the model to be updated every time new data comes in and accommodate the changes in an effective way.
% % like humans' ability to continually acquire, update, and accumulate knowledge in response to external environmental change.
% For instance, a deployed self-driving system needs to be updated when new training data is available to adapt to more driving scenarios.
% % language modeling systems need to be updated regularly to reflect the new changes and developments happening in the world. 
% How to maximize the performance of the model with the latest data becomes one of the essential problems that needs to be addressed. 


% The common approach to updating the model is to train the model from scratch with all the available data every time new data arrives. However, this undermines the benefit of leveraging the learned knowledge and leads to large train costs. It is also not practical in storage-limited systems where storing all past data is not feasible.
% One natural way then to consider is to train the model with the new data, starting with the initialization from the latest checkpoint. 
% % While such a ``warm-start'' initialization makes sense to leverage what has been learned in the past, 
% However, it has been observed in prior work that such ``warm-starting'' hurts the generalization of deep neural networks compared to random initialization~\cite{ash2020warm, achille2017critical, caccia2022anytime}. 
% % This also happens in online active learning, where people solve it by simply training the model from scratch. 
% % Therefore, improving the generalization of warm-started models plays an essential role in models' continuous improvement and adaptation. 
% Among the existing methods, inheriting selective learned knowledge from the learned model during initialization~\cite{ash2020warm, ramkumar2023learn, taha2021knowledge, zhou2022fortuitous} and adding certain regularizations~\cite{shon2022dlcft} are the most popular and have shown efficacy for accuracy improvement. 

% The data collected in the past can be accessible or not accessible in different practical applications. In storage-limited systems with no access to past data, the model suffers severe catastrophic forgetting when training on new data. 
% % the problem becomes more like a data-incremental continual learning problem where the model needs to accommodate new information while remembering the learned knowledge. 
% Many continual learning methods have been proposed to mitigate forgetting~\cite{de2021continual, zhou2023deep}.
% However, existing continual learning approaches mostly aim at task-incremental or class-incremental situations~\cite{wu2019large, kirkpatrick2017overcoming, gao2023unified, yan2021dynamically, luo2023class}, and we empirically find that they fail to work well in the data-incremental setup which has been rarely explored. This is intuitively explainable: In class or task incremental problems, the model has converged fully on previous classes as it assumes all the related data samples are provided at once in the corresponding round.
% % When moving the next task or classes, the key is to maintaining the accuracy on old ones while adapting to new knowledge. 
% So typical methods aim at staying as close as possible to the prior solution~\cite{kirkpatrick2017overcoming}. However, in general data-incremental, the accuracy of all classes has potential to improve given more data samples, thus requiring the model to move away from the previous convergence point learned from limited data and seek a trade-off between learning and forgetting. 
% % Such a nuance suggests the need for an exploration of this common but rarely-studied problem. 
% Knowledge distillation~\cite{gou2021knowledge} is also one of the widely applied approaches to transfer the learned knowledge to the model being trained~\cite{madaan2023heterogeneous, iscen2020memory, li2017learning, dhar2019learning}. In the data-incremental case, however, the previously trained models tend to be weak teachers as they are trained with less data. This poses additional challenges to the knowledge transfer so that the teacher does not over-guide the student~\cite{lee2023study}.



% In this paper, we restrict the problem to data-incremental with stationary distributions and study the solution to train a warm-starting model with incremental data. For a model to be improved with new data, we propose to first step out of the previous convergence point and seek a better one. This actually also aligns with the effect of methods proposed in prior literature for model generalization improvement~\cite{ash2020warm, ramkumar2023learn, zhou2022fortuitous}, where they select heritage partial of learned knowledge allowing a better loss landscape exploration. 

% Then we propose to apply a novel feature regularization (FeatReg) to retain knowledge and refine the learned feature representation in both scenarios where the past data is accessible and not accessible. For the latter scenario, we also propose to apply adaptive knowledge distillation (AdaKD) for knowledge transfer from the weak teacher. We test our algorithm with large-scale dataset ImageNet~\cite{imagenet} and show the efficacy of our method. We also show that our method is compatible with other orthogonal approaches and the combination brings higher accuracy.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


A common real-world setting involves data that are being provided to the machine learning system in
a stream

 At every step, the learner is given k new samples to append to its training data, and it updates
its hypothesis to reflect the larger dataset.


In this section we provide empirical evidence that warm starting consistently damages generalization
performance in neural networks.
The model is trained to convergence on the first
half, then is trained on the union of the two batches, i.e., 100\% of the data

Even though MLP and ResNet optimization is non-convex, conventional
intuition suggests that the warm-started solution should be close to the full-data solution and therefore
a good initialization. One view on pre-training is that the initialization is a “prior” on weights; we
often view prior distributions as arising from inference on old (or hypothetical) data and so this sort
of pre-training should always be helpful. The generalization gap shown here creates a computational
burden for real-life machine learning systems that must be retrained from scratch to perform well,
rather than initialized from previous models



We simulate this paradigm 



 We examine two cases: 
1) where the model is retrained
from scratch after each batch, starting from a random initialization, and 2) where the model is trained
to convergence starting from the parameters learned in the previous iteration. In both cases, the
models are optimized with Adam, using an initial learning rate of 0.001. Each was run five times with
different random seeds and validation sets composed of a random third of available data, reinitializing
Adam’s parameters at each step of learning

s of training, and while it is helpful,
regularization does not resolve the generalization gap induced by warm starting


Our experiments show that applying the same
amount of regularization to randomly-initialized models still produces a better-generalizing classifier.


when new samples are appended to the training set, we propose initializing the network’s
parameters by shrinking the weights found in the previous round of optimization towards zero, then
adding a small amount of parameter noise. 


Practitioners have then to decide how to allocate their computational budget in order to obtain the
best performance at any point in time.

As future steps, when and how do we need to incorporate these data points to the training process. 


Empirically, 
